Non-Parametric Calibration of Probabilistic Regression

The task of calibration is to retrospectively adjust the outputs from a machine learning model to provide better probability estimates on the target variable. While calibration has been investigated thoroughly in classification, it has not yet been well-established for regression tasks. This paper considers the problem of calibrating a probabilistic regression model to improve the estimated probability densities over the real-valued targets. We propose to calibrate a regression model through the cumulative probability density, which can be derived from calibrating a multi-class classifier. We provide three non-parametric approaches to solve the problem, two of which provide empirical estimates and the third providing smooth density estimates. The proposed approaches are experimentally evaluated to show their ability to improve the performance of regression models on the predictive likelihood.

==> notation_list.tex <==
\begin{landscape}
\section*{Notation List}

\begin{table}[h]
    \centering
    \begin{tabular}{|l|l|l|l|}
    \hline
    & Binary Classification & Multi-class Classification & Regression \\
    \hline 
    Feature space & \multicolumn{3}{l|}{$\mathbb{X}$} \\
    \hline
    \dots random variable & \multicolumn{3}{l|}{$\mathbf{X}$} \\
    \hline
    \dots instance & \multicolumn{3}{l|}{$\mathbf{x}$} \\
    \hline 
    Target space & $\mathbb{Y} = \{+,-\}$ &  $\mathbb{Y} = \{1,2,...,K\}$ &  $\mathbb{Y} = \mathbb{R}$ \\
    \hline
    \dots  random variable & \multicolumn{3}{l|}{Y}\\
    \hline
    \dots  instance & \multicolumn{3}{l|}{$y$}\\
    \hline
    Probabilistic output space & $\mathbb{S} = [0, 1]$ & $\mathbb{S} = \Big\{[s_1, s_2, ..., s_K] \mid \sum_{i=1}^{K}s_i = 1, s_i \geq 0 \Big\}$ & $\mathbb{S} = \Big\{ \mathsf{s} \mid \mathsf{s}: \mathbb{R} \rightarrow [0, +\infty), \int_{y=-\infty}^{+\infty} \mathsf{s}(y) \: dy = 1 \Big\} $ \\
    \hline 
    \dots  random variable & S & $\mathbf{S} = [S_1,...,S_K]$ & $\mathsf{S}$\\
    \hline
    \dots  instance & s & $\mathbf{s} = [s_1,...,s_K]$ & $\mathsf{s}$\\
    \hline
    Cumulative probabilistic output space & $\mathbb{Q} = [0, 1]$ & $\mathbb{Q} = \Big\{ [q_1,...,q_{K-1}] \mid q_i \leq q_{i+1}, 0\leq q_i \leq 1 \Big\}$ & $\mathbb{Q} = \Big\{ \mathsf{q} \mid \mathsf{q}: \mathbb{R} \rightarrow [0,1], \mathsf{q}(t) = \int_{y=-\infty}^{t} \mathsf{s}(y) \: dy, \mathsf{s} \in \mathbb{S} \Big\}$ \\
    \hline
    \dots  random variable & Q & $\mathbf{Q} = [Q_1,...,Q_{K-1}]$ & $\mathsf{Q}$\\
    \hline
    \dots instance & q & $\mathbf{q} = [q_1,...,q_{K-1}]$ & $\mathsf{q}$ \\
    \hline
    \end{tabular}
    \caption{List of notations (spaces, variables, and instances) }
    \label{tab:list_of_notations_1}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{|l|l|l|l|l|}
    \hline
    & Binary Classification & \multicolumn{2}{l|}{Multi-class Classification} & Regression \\
    \hline 
    \multirow{2}{*}{Soft} & \multirow{2}{*}{$\mathsf{f} : \mathbb{X} \rightarrow \mathbb{R}$} & 1 v.s. 1 & $\mathsf{f} : \mathbb{X} \rightarrow \mathbb{R}^{K \cdot (K-1) / 2}$  & \multirow{2}{*}{NA} \\
     &  & 1 v.s. rest & $\mathsf{f} : \mathbb{X} \rightarrow \mathbb{R}^{K}$ &  \\
    \hline
    Probabilistic & $\mathsf{f}: \mathbb{X} \rightarrow [0,1]$ &  \multicolumn{2}{l|}{$\mathsf{f}: \mathbb{X} \rightarrow \Big\{[s_1, s_2, ..., s_K] \mid \sum_{i=1}^{K}s_i = 1, s_i \geq 0 \Big\}$} & $\mathsf{f}: \mathbb{X} \rightarrow \Big\{ \mathsf{s} \mid \mathsf{s}: \mathbb{R} \rightarrow [0, +\infty), \int_{y=-\infty}^{+\infty} \mathsf{s}(y) \: dy = 1 \Big\}$  \\
    \hline 
    Hard (Crisp) & $\mathsf{f} : \mathbb{X} \rightarrow \{+, -\}$ & \multicolumn{2}{l|}{$\mathsf{f} : \mathbb{X} \rightarrow \{1, 2, ..., K\}$} & $\mathsf{f}: \mathbb{X} \rightarrow \mathbb{R}$\\
    \hline
    \end{tabular}
    \caption{List of Notations (Functions) }
    \label{tab:list_of_notations_2}
\end{table}
\end{landscape}

